Insights into Chemical and Structural Order at Planar Defects in a Functional Oxide Using Multislice Electron Ptychography

Switchable order parameters in ferroic materials are essential for functional electronic devices, yet disruptions of the ordering can take the form of planar boundaries or defects that exhibit distinct properties. Characterizing the structure of these boundaries is challenging due to their confined size and three-dimensional nature. Here, a chemical anti-phase boundary in the highly ordered double perovskite \ce{Pb2MgWO6} is investigated using multislice electron ptychography. The boundary is revealed to be inclined along the electron beam direction with a finite width of chemical intermixing. Additionally, regions at and near the boundary exhibit antiferroelectric-like displacements, contrasting with the predominantly paraelectric matrix. Spatial statistics and density functional theory calculations further indicate that despite their higher energy, chemical anti-phase boundaries form due to kinetic constraints during growth, with extended antiferroelectric-like distortions induced by the chemically frustrated environment in the proximity of the boundary. The three-dimensional imaging provides critical insights into the interplay between local chemistry and the polar environment, elucidating the role of anti-phase boundaries and their associated confined structural distortions and offering new opportunities for engineering ferroic thin films.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
